Adversarial Unsupervised Representation Learning for Activity Time-Series

Sufficient physical activity and restful sleep play a major role in the prevention and cure of many chronic conditions. Being able to proactively screen and monitor such chronic conditions would be a big step forward for overall health. The rapid increase in the popularity of wearable devices provides a significant new source, making it possible to track the user's lifestyle real-time. In this paper, we propose a novel unsupervised representation learning technique called activity2vec that learns and "summarizes" the discrete-valued activity time-series. It learns the representations with three components: (i) the co-occurrence and magnitude of the activity levels in a time-segment, (ii) neighboring context of the time-segment, and (iii) promoting subject-invariance with adversarial training. We evaluate our method on four disorder prediction tasks using linear classifiers. Empirical evaluation demonstrates that our proposed method scales and performs better than many strong baselines. The adversarial regime helps improve the generalizability of our representations by promoting subject invariant features. We also show that using the representations at the level of a day works the best since human activity is structured in terms of daily routines

==> sections/problemstatement.tex <==
%In this section, we describe our problem, provide insights into the unique challenges and properties of human activity data.



%\subsection{Problem Setting}
Wearables data has created new opportunities to understand how human behaviors such as physical activity and sleep affect our cognitive and physical health. This is especially important given that there are millions of users of wearable devices.
Additionally, consumers have started tracking their own activity on the web using personal health web applications \cite{fernandez2013free} like Microsoft HealthVault or \textit{GoogleFit} as shown in Figure~\ref{fig:workflow}. Some users even provide access to  their Electronic Health Records (EHRs)~\cite{yadav2015mining} for health studies, providing a rich source of information. This data can be utilized by health-care providers as well as consumer electronic companies to help screen subjects for early detection of disorder conditions~\cite{fitcancer}, real-time lifestyle recommendations, and monitoring lifestyle therapy compliance~\cite{yom2017encouraging}.

%\subsection{Challenges and Opportunities}

With the opportunity for understanding the connection between human activity and sleep patterns using wearables technologies, we address the following challenges:

\begin{noindlist}
\item \emph{Limited availability of EHR diagnosis data:} Diagnosis information is only available for a few users who allow access to EHRs for health-care providers or application providers. In such a scenario, we have a very limited fraction of users whose both wearables  data  as well as diagnosis information is available. Using a purely supervised learning approach renders the activity data from other users redundant. This necessitates an unsupervised or semi-supervised learning approach that can exploit the larger pool of `unlabeled' activity data coming from wearable devices.  
%\item \emph{Exploiting Co-morbidity:} Many disorders are inter-related, with one impacting the other or vice-versa. Caused by common life-style  choices or genetic risks, such mutually co-occurring (and usually correlated) health conditions are referred to as co-morbidity~\cite{berndt1994using}. To exploit this correlational structure, and better understand life-style choices (activity patterns) leading to such outcomes, it is important to jointly learn the models for risk assessment from activity data. 
\item\emph{Generality of learned models:} Due to sample skews of populations in the survey data and subject specific conditions,  algorithms developed using only labeled data might not work well with the general population.  In addition, it is also common that general purpose wearable analytics perform poorly in cohorts of people with chronic conditions (\eg\ underestimating steps) \cite{storm2015step}. Hence, an unsupervised learning algorithm that mines the activity patterns rather than doing an end-to-end learning is desirable.
\end{noindlist}


%We propose \acttovec\, an unsupervised learning algorithm for activity time-series for addressing problems (1) and (3). Our multi-task learning approach exploits (2) for better performance on disorder detection tasks from wearables data. We describe our models in next section.


%A major problem is that curated health datasets are available (e.g. www.sleepdata.org) but often those are heavily biased towards particular populations with particular health problems. Consequently, algorithms developed using those datasets might not work well with the general population. In addition, it is also common that general proposes wearable analytics do perform very badly in cohorts of people with chronic conditions (e.g.  underestimating steps) \cite{storm2015step}. This is mainly caused because algorithms for analyzing the wearable data are designed for specific subpopulations and consequently perform badly with more general populations. This problem will be a major roadblock to take advantage of the mass amounts of wearable data which is being collected both in consumer (e.g. \cite{fagherazzi2017international}) and clinical settings (e.g. \cite{wright2017analysis}).   In this study we present a multi-task learning approach to analyze health problems across various and heterogeneous data sets. 



%\subsection{Problem Statement}
%With an increasing popularity of wearable devices we have an enormous ability to track human physical activity and sleep in real-time. It is essential to leverage such valuable data for detecting of early signs of health problems and enhancing strategies for health prevention both at the population and individual level. Physical activity is an influenced and influencing many health aspects, but it is a parameter very hard to quantify and measure without the use of objective data collection from devices such as fitness and sleep trackers. For example, we know that lack of sleep can lead to hypertension \cite{palagini2013sleep}, but it is hard to understand how physical activity and sleep do play a role in the pathophysiological mechanisms underlying all these lifestyle factors. It is known that properly addressing lifestyle factors we can prevent 8 out of 10 chronic conditions, and this has lead to the development of lifestyle medicine as a potential solution \cite{sagner2014lifestyle}. Analytics can allow patients and professional to act quicker towards identifying lifestyle changes that might be negatively impacting health.  In such a scenario, it is of enormous value to be able to predict possible health changes a subject might be suffering from in an automated real-time manner by utilizing the time-series data.

%\paragraph{Challenges:} The major issues, however, are \textbf{absence} of diagnosis data of subjects, representative of the data due to biased datasets with (i.e. population skew) (age, disorder population) of subjects, and the noisy nature of measurements related to physical activity and sleep. In such a setting it is important to use unsupervised learning methods to generalize, rather than a narrow focus of end-to-end supervised learning.

%\paragraph{Unique properties of human activity data}

